Violet: A Vision-Language Model for Arabic Image Captioning with Gemini Decoder

Although image captioning has a vast array of applications, it has not reached its full potential in languages other than English. Arabic, for instance, although the native language of more than 400 million people, remains largely underrepresented in this area. This is due to the lack of labeled data and powerful Arabic generative models. We alleviate this issue by presenting a novel vision-language model dedicated to Arabic, dubbed \textit{Violet}. Our model is based on a vision encoder and a Gemini text decoder that maintains generation fluency while allowing fusion between the vision and language components. To train our model, we introduce a new method for automatically acquiring data from available English datasets. We also manually prepare a new dataset for evaluation. \textit{Violet} performs sizeably better than our baselines on all of our evaluation datasets. For example, it reaches a CIDEr score of $61.2$ on our manually annotated dataset and achieves an improvement of $13$ points on Flickr8k.

==> Dataset.tex <==
% \section{Data Collection}
% None of the previous works on Arabic captioning released their training data, so we first started by creating a training dataset for our model. Since manually labeling and creating a new dataset is both time-consuming and expensive, we opted for translating the commonly used captioning dataset Microsoft Common Objects in Context (MSCOCO). There are two famous training/validation splits for this dataset, the 2014 Karpathy's split, and the 2017 split. Both splits contain the same images and only differ in the split ratio. The dataset covers around 80 different objects in a total of 123k images with an average 5 captions per image. The dataset was annotated by humans, which makes it a suitable dataset for evaluation. We created our dataset in two stages, Translating the dataset, and then filtering poor translations.
% % Since there were no reliable Arabic captioning datasets our first obstacle was to create such datasets. We started by collecting common English captioning datasets such as CoCo, CC3M, SBU, ..etc. We Then compared the output google translate API \cite{} with Meta's No Language Left Behind (NLLB) \cite{costa2022no} model, and after manually checking ht outputs and comparing the perplexity of both models, we decided to stick with NLLB for translation.

% \subsection{Machine Translation}
% In all of the previous attempts at arabic image captioning pretraining\cite{eljundi2020resources}\cite{emami2022arabic}\cite{lasheen2022arabic}, google API was used for translating the datasets \cite{google}. Despite that, the quality of the translations is not good enough. The authors in \cite{sabri2021arabic} reported that from a random sample a whooping 46\% of the translation obtained by Google API were unintelligible. Motivated by that, we  decided to investigate meta's no language left behind model (NLLB) \cite{NLLB} for translation.


% We conducted the comparison on two ~metrics~, first was to manually check the quality of 200 sentences translated by both models. While the second was to calculate the perplexity of the translations using our Jasmine decoder. Perplexity calculates 
% Our observation was Google API tends to have literal translation compared to NLLB, empirically, we found that 42\% of Google translations to be unintelligible compared to only 15\% from NLLB, this aligns with the findings in \cite{ACL}. We also compared with chatgpt which only had 7\% error rate in the translation, but we opted for NLLB since it was open source.
% \subsection{Filtering Process}
% Despite NLLB having better translations compared to that of Google API, instances of noise and poor translations in the output. Moreover, as shown in Figure, our manual inspection revealed that certain English captions in the original dataset were also noise. To mitigate this issue, we employed semantic similarity techniques.
% Semantic similarly gives an idea of how close the meaning of two sentences is, by comparing their embeddings.
% % More concretely, the embedding of both sentences is obtained and a similarity metric, such as cosine similarity, is used to evaluate how similar the two embeddings are. The smaller the angle between the two vectors the higher the larger the similarity score is and the more close the sentences are. 

% In our experiments, we used sentence BERT \cite{sentence_bert} to calculate the semantic similarity between each caption and its translation. 
% After obtaining the embeddings using BERT, cosine similarity is calculated between the two sentences where higher values indicate a smaller angle between the embeddings vector which means higher similarity and vice versa. We empirically choose a threshold value of 0.8 and rejected all captions with lower similarity. This resulted in removing a total of 50K samples from the whole dataset. 
% %495736 train, 22845 val and 22912 test


==> Results.tex <==


\section{Results and discussion}
In this section .. 

% \begin{table*}[htp]
% \centering

% \begin{tabular}{p{3.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{0.5cm}p{1.5cm}p{1.5cm}p{1.5cm}}%{lccccccccccc}
% \toprule
% \multirow{3}{*}{Method} & \multicolumn{3}{c}{\emph{$Flickr8k$}} && \multicolumn{3}{c}{\emph{$CoCo$}}\\
% \cmidrule{2-4} \cmidrule{6-8}
% & Belu4 $\uparrow$  & Rouge $\uparrow$ & CIDER $\uparrow$ && Belu4 $\uparrow$ & Rouge $\uparrow$ & CIDER $\uparrow$\\
% \midrule
% \midrule
%     CNN-LSTM \cite{al2018automatic}  & 8 & -& - & -& - & -& -\\
%     LSTM \cite{lasheen2022arabic}  & 27.12 & -& - & & 12.50 & -& -\\
%     LSTM & - & -& - & -& - & -& -\\
   
%     \midrule
%     \rowcolor{blue!6} \textbf{ (transformer)} & - & -& - & -& - & -& -\\
%     \rowcolor{blue!6} \textbf{ (transformer)} & - & -& - & -& - & -& -\\
%     \rowcolor{blue!6} \textbf{ VisualGPT} & - & -& - & -& 11.2 & -& 72.31\\
%     \rowcolor{blue!6} \textbf{ VASMINE(default)} & - & -& - & -& 13.41 & 26.37& 53.22\\
%     \rowcolor{blue!6}\textbf{ VASMINE(Gemini)} & - & -& - & -& 25.21 & 46.64& 83.33\\
    
%   \bottomrule
% \end{tabular}
% \caption{bla bla bla}
% \label{table_small}
% \end{table*}


==> eval.tex <==
\section{Experiments and Evaluations}\label{expr}
\subsection{Data}
\subsection{Data Augmentation}
\subsection{Model Configuration and Settings}
\subsection{Results}

==> expr.tex <==
\section{Experiments and Evaluations}\label{expr}
\subsection{Data}
\subsection{Data Augmentation}
\subsection{Model Configuration and Settings}
\subsection{Results}

==> literature.tex <==
\section{Related Works}\label{RW}
\subsection{Traditional Approaches}
HMMs, CTC and RNNs Models
\subsection{Transformers-based  Approaches}
Transformers stuffs 



\section{Vision-Language Models}
Vision language models (VLMs) can be categorized into multiple categories based on different criteria.The first criterion is whether the vision encoder output comprises only image features or region features from an image detector. The second criterion is the architecture of the language part, which can be either encoder-only, decoder-only or encoder-decoder. Finally, the attention mechanism used to integrate the visual and linguistic information, which can either cross-attention or merged attention.
In this section, the most recent architectures in VLMs are going to be discussed, following the aforementioned attention mechanism categorization criteria. More emphasis will be put on the different tweaks added in each architecture and the different training objectives proposed in each.





% Majority of recent vision language models (VLMs) can be categorized under two main categories based on their attention mechanism for integrating vision and language information. The first category is cross-attention, where the query is obtained from the language side, while the key and value pairs are obtained from the vision side. On the other hand for merged attention, both the visual and language tokens are concatenated and passed through the same decoder.
% This section discusses the most recent architectures under both categories, stressing on the different tweaks and training objectives proposed in each.
\subsection{Cross-attention Based Architectures}
In cross-attention, commonly, the query vector is obtained from the language side, while the key and value pairs are obtained from the vision side. The main reason for that is, text is more natural way to guide the attention of the model, while visual information are typically more complex. Following are the most recent models employing this mechanism.
\subsubsection{Flamingo: a Visual Language Model for Few-Shot Learning}
Flamingo was the first model to introduce the approach of having a text interleaved by images as an input for VL models. The model architecture consists of a frozen image encoder, a preciever resampler, a frozen text decoder with cross-attention layers, and a gating mechanism. The image encoder is a frozen Free ResNet(NFNet)\cite{brock2021high} architecture which is trained on a contrastive image objective\cite{radford2021learning}, the output of the image encoder is passed to a trainable perceiver resampler in order to reduce computational complexity. The text decoder is a frozen Chinchilla model with cross-attention layers inserted between its layers, a tanh gating mechanism is used in order to keep the language model fluency intact while initialization the new cross-attention layers. This allows for improved stability and performance.

As mentioned before, the input to the model is a text interleaved by images. In order to pass it as input to the model, it first need preprocessing. A special token <image> replaces each image position in the input and an <|endofchunk|> token is placed after each text chunk before an image. The model training objective is an auto-regressive language modeling task, where the model predicts the next work given the previous predicted words and image. The cross-attention is only applied on the image just before each interleaved text sequence instead of being applied on all the previous images. The datasets used are: M3W which a massive dataset of interleaved image and text scrapped from the web, ALGIN dataset \cite{jia2021scaling} and a dataset of video and text pairs.

The model performs really well on a wide range of VL tasks even in few shots setting including, image captioning, video question answering, visual question answer, visual reasoning and many more. The input is appended with a prompt to specify the intended task, for example: in case of VQA the input would be something like "<image> Question: <text>? Answer:" or for case of captioning "<image>Output:" the model then generates the output given this input.

\subsubsection{CoCa: Contrastive Captioners are Image-Text Foundation Models}
CoCa is a text-decocder and image-encoder architecture that decouples the text decoder into two equal parts: a vanilla decoder and a decoder with cross-attention layers. The first part of the decoder serves as a unimodal text encoder and the second part functions as multi-modal decoder. Prior to passing the output of the vision encoder through cross-attention, the output is passed through a multi-head attention layer which acts as an attention pooler. The attention pooler have a learable query matrix that learns to extract more refined visual information. The model is trained from scratch on two pretraining objectives. The first objective is contrastive learning, where the class token of the vision encoder and the uni-modal text part of the decoder is used to maximize the similarity between each image and its caption while also minimizing the similarity with every other caption and vice versa. The second training objective is the auto regressive language modeling objective.

The model is trained on two dataset. The first dataset is ALIGN \cite{jia2021scaling}, which is a large scale dataset with noisy alt-texts. While the second data set is JFT-3B, which is original a massive image classification dataset. to adapt this dataset for the training objective, the image labels are treated as captions..
Coca achieves state of the art performance on multiple benchmarks including VQA, image captioning and image classification.

\subsubsection{OFA: UNIFYING ARCHITECTURES, TASKS, AND MODALITIES
THROUGH A SIMPLE SEQUENCE-TO-SEQUENCE LEARNING
FRAMEWORK}
OFA \cite{} is an image encoder and a text decoder based architecutre that aims at having a unified model to perform both uni-modal and multi-modal tasks. The model uses a ResNet as the image encoder and a vanilla decoder as the text decoder with cross-attention layers. The visual features are reduced in size via sparse decoding \cite{bao2021beit}, textual data is tokenized using byte-pair encoding (BPE). Objects, which needed for tasks such as visual grounding, are also represented as sequence of discrete tokens. The object labels are represented as text tokens, using BPE, and coordinates are discretized to integers tokens (top-left and bottom-right coordinates). 

The model is trained on public  uni-modal and cross-modal datasets including: Pile (language), OpenImages (vision), YFCC100M (vision), CC12M \cite{}, VQAv2 and RefCOCO. The model is trained in a languge modeling task manner where given the predicted tokens, the model predict next ones. 


\subsubsection{VisualGPT: Data-efficient Adaptation of Pretrained Language Models for Image Captioning}
VisualGPT \cite{chen2022visualgpt} is an efficient vision encoder text fusion decoder that performs very well with little training data. The model architecture follows that of meshed transformer \cite{cornia2020meshed}, with two main differences: employing a pretrained language model, and using a gating mechanism to balance the contribution of the language and vision parts. 

Meshed transformer adds two modifications to the transformer architecture: first it makes connection between each encoder layer too to each decoder layer, instead of only using the output of the last encoder layer. Furthermore, since the model uses detection regions instead of image, they propose adding learnable vectors they called memory, to the keys and values, to further capture knowledge about the relation between the regions.
%##############################################
Similar to \cite{cornia2020meshed}, in the vision encoder, the key and value are extended with additional learnable vectors called memory. Since the model uses detection regions, self-attention would be sub-optimal at encoding the relation between these regions for cross-attention. These memory vectors are expected to encode prior knowledge about the relationships between the regions.
%##############################################
In order to stabilize the training of the cross-attention layers with the pretrained language model layers and avoid overwriting pretrained weights, a gating mechanism called self-resurrecting activation units is used. The gate allows gradient of every element of either the language self-attention or the cross-attention to flow according to a certain threshold. If any element is below that threshold, its gradient is set to zero. More concretely,
EQ

The model achieves a competitive performance in image captioning with little training data. But this performance gain decreases against other models when more training data is available. 

\subsubsection{BLIp-2}
BLIP-2 follows the direction of reducing the dimensionality of the input visual features by extracting only the most significant information. The model achieves this by learning latent input queries through the integration of a transformer architecture named Q-former. This transformer block consists of two sub-parts, an image transformer and a text transformer with shared self-attention. The image transformer is a stack of transformer blocks with a cross-attention layer every other block, the input to the cross-attention is a frozen image encoder output and the learnable latent queries after passing through the self-attention layers. The text transformer can act as a text encoder and a decoder by adding a prefix to the input, and similarly, it is a stack of transformer blocks. Clip ViT/14L is used as the image encoder and the Q-former is initialized with $BERT_{base}$ weights (the cross-attention layers and latent queries are randomly initialized)

The training is done on two stages: The first stage focuses on learning the latent queries from frozen image encoder, while the second stage make use of a pretrained large language model to give generative capabilities to the architecture.
The first pretraining stage consists of three training objectives where the only trainable component is the Q-former and the latent queries. The first training objective is Image text contrastive learning where the similarity between the output of the latent queries and the output of the CLS token of the text decoder is computed and the highest similarity is chosen as the image-text similarity. The second training objective is Image-grounded text generation which uses masked self-attention where the text decoder predicts the next token given the latent queries and the generated words so far. The last training objective of the first stage is Image-Text matching, where the output of the latent queries is fed to a binary classifier to predict whether image-text pair are matching or not.
For the second pretraining stage, the model from the first stage is passed through a fully connected layer and is fed as an input to a large language model. Both the image encoder and the language model are frozen, while the Q-former and the Fully connected layer are trainable. The training objective is a next token prediction task, where the latent query is used as either a prior or a prefix to the input text.
%Maybe call merged attention models decoder a fusion decoder?
\subsection{Merged-attention Based Architectures}
Merged-attention concatenate both the visual and linguistic tokens into one vector and use the vanilla self attention. Although this allows for better communication and attending between the vision and language side, the information extracted from the tokens is not as rich as cross-attention. Following are the most recent models employing this mechanism.
\subsubsection{Learning Transferable Visual Models From Natural Language Supervision }
CLIP \cite{radford2021learning} is one of the early very successful methods at aligning visual and linguistic features. The reason behind the method was the scarcity of manually annotated data and the ease of obtaining image-language pair data from the internet. The model is trained on Coco, visual genome, cleaned version of YFCC100M as well as a newly created dataset called WebImageText(WIT). 
The architecture used is a vanilla ViT\cite{dosovitskiy2020image} and a vanilla text decoder \cite{vaswani2017attention} trained from scratch. The $[$ cls $]$ token at the output of the image encoder is treated as the visual features, while the $[$ EOS $]$ token in the text decoder is treated as the textual features.

For the model training, Instead of following the mainstream predictive objective where the model predicts the input text describing the image, the authors opted for the more efficient contrastive approach. The training objective is to maximize the similarity between each image and its sentence while minimizing the similarity with all other captions. This is achieved by maximizing the cosine similarity for the positive pair  of the linearly projected and normalized visual features with the linearly normalized and projected textual features and minimizing it with all other negative pairs. Where symmetric cross-entropy loss is used on top of these similarities.  

In order to use the model for zero-shot classification the input of the model is manipulated to follow that of the training objective. Each input image is compared with the text representing each of the classes in the form of "A photo of a \{object\}" where "object" is the label of each class. Then, the similarity between the image and each sentence is computed and the largest similarity is considered to be the correct prediction.




\subsubsection{Oscar: Object-Semantics Aligned Pre-training for Vision-Language Tasks}
Oscar\cite{li2020oscar} is an encoder-only based model that integrates the usage of object tags (labels) as an input to the transformer in addition to textual and visual inputs. The encoder is a pretrained BERT \cite{devlin2018bert}, which takes a triplet consists of the word sequence tokens, object tags tokens and region features tokens as an input. Object tags and region features are extracted using Faster R-CNN, where the object tags uses the same vocabulary of the text.

The model has two pre-training objectives: masked token loss and contrastive loss. The masked token loss is similar to BERT's masked language modeling, where at each iteration each token in the linguistic part (both the text and tags) is masked with a certain probability, and the goal is to predict the masked tokens given surrounding tokens and all the visual features. On the other hand, for contrastive loss the tags and images features are treated as the image modality, the descriptions are the language modality. A “polluted  image” is created by replacing the object tags  by a 50\% probability with a different tags sequence randomly sampled from the dataset. A fully connected layer is used on top of the [CLS] token for classification (correct pairs or not). The final pre-training loss is calculated as follows:

EQ

Oscar performs well on several downstream tasks including, Image-Text Retrieval, Image captioning (treats the encoder as an auto-regressive architecture by appending mask token auto-regressivly), novel object captioning, VQA, GQA, and Natural Language Visual Reasoning for Real (NLVR2).

\subsubsection{GIT: A Generative Image-to-text Transformer for Vision and Language}
GIT uses a basic approach consists of a text decoder and a vision encoder. The image encoder is the swin-like \cite{liu2021swin} architecture Florence \cite{yuan2021florence} which is pretrained in contrastive manner. The the text decoder, however, is a randomly initialized vanilla transformer decoder.
The model employs merged attention, which is suggested to provide better performance than cross-attention for large-scale pretraining. The pre-training objective is an auto-regressive language modelling task, which involves predicting the next word in a sentence based on the image features and any preceding words. The model was trained on a dataset of 0.8 billion image-text pairs. 



GiT achieves competitive performance on several downstream tasks such as image captioning, video captioning, VQA, OCR and even image recognition. In case of image captioning the model utilizes the same input as in pretraining. While for VQA task, the image features, the question and the ground truth answer are concatenated, but the objective loss is only applied on the answer tokens. The answer is generated in an auto-regressive manner, unlike most previous works that treated VQA as a classification task. Similarly, OCR capabilities are achieved as a byproduct of the large scale pretraining, enabling the model to answer text related questions in the image. Finally, for image classification, the model generates the class labels as an image caption, this is different from previous works since there is no predefined labels for the classes.

\subsubsection{SIMVLM: SIMPLE VISUAL LANGUAGE MODEL PRETRAINING WITH WEAK SUPERVISION}
SimVLM \cite{wang2021simvlm} is an image encoder and text decoder based architecture that utilizes both multi-modal and text training data. The model is trained end-to-end from scratch using prefix language modeling as a single training objective. Similar to vanilla auto-regressive language modeling, prefix language modeling randomly samples a chunck of text that is concatenated to the visual tokens and passed through the transformer decoder. Given the image tokens and the chunk of text, the model auto-regressively generate the next tokens following this equation:
EQ

Thanks to the aforementioned training objective, the model can utilize multi-modal inputs as well as text only inputs. Specifically, the model is trained on the noisy image-text pairs dataset ALIGN \cite{jia2021scaling} as well as the large scale text dataset  Colossal Clean Crawled Corpus (C4) \cite{????}. After pretraining the model is evaluated in zero-shot setting several downstream benchmark tasks including: Visual question answering, Visual Entailment, Natural Language Visual Reasoning, Image Captioning and Multimodal Machine Translation. The authors argued that adding the prefix "A picture of", in case of image captioning, improved the model performance. For some downstream tasks, such as Visual Entailment, the model is fine tuned on text only data.


\subsubsection{VLMO: Unified Vision-Language Pre-Training with Mixture-of-Modality-Experts}
VLMO follows a different approach to the text encoder vision encoder based architecture. The authors introduce the concept of Mixture-of-Modality-Experts (MoME), where a single encoder is trained in order to be used as a text encoder, image encoder and vision language encoder. This is achieved by creating a pool of modality specific experts in the form of feed-forward networks (FFN), in each transformer block while sharing all other parameters in the attention layers.

Concretely, the model is trained over three stages in the following order: with visual data only (vision encoder), with textual data only (text encoder) and with multi-modal data (fusion encoder). For the vision encoder, the transformer encoder is initialized with the pretrained parameters of BEiT \cite{bao2021beit} and, similarly, the model is trained following the same masked image modeling task.
While for the text encoder, a new FFN is added in each transformer block while freezing all other network parameters (self attention layers and previous vision encoder FFN). The model is trained on the vanilla masked language modeling task of BERT \cite{devlin2018bert}. Finally, for the fusion encoder in the first half of the transformer the vision FFN and the text FFN takes their respective modality from the output of each transformer block. While in the second half, a new FFN is initialized to act as the multi-modality encoder.

In the last training stage with the multi-modal data, all the parameters of the transformer are trainable. The training objectives for the final pretraining stage are image-text contrastive learning and image-text matching.  In case of image-text contrastive objective, the class tokens appended to the visual and textual input, [I\_CLS] and [T\_CLS], are used as representation for the image and text inputs. And the similarity between the image and text are calculated by comparing the feature vector of both class tokens after being linearly projected and normalized. The vanilla contrastive image-to-text and text-to-image loss is calculated using cross-entropy. For the image-text matching task, the model needs to predict whether a caption belongs to the given image or not. The samples for this loss are chosen via hard negative mining from the contrastive objective and the text class token [T\_CLS] is used for the prediction. 
The training datasets used are Conceptual Captions, SBU Captions, COCO and Visual Genome.

\subsubsection{Pixel-BERT: Aligning Image Pixels with Text by Deep Multi-Modal Transformers}
Pixel-BERT is a vision encoder and a fusion encoder based architecture that uses image features rather than image patches or detection regions. The vision encoder is an image pretrained CNN, while the fusion encoder is a BERT \cite{devlin2018bert} pretrained transformer encoder. Similar to BERT, the textual input is tokenized using WordPiece, mapped into a embedding matrix and added to a positional embedding. On the other hand, the visual features extracted using the CNN are added to a semantic embedding vector in order to differentiate them from the textual inputs. The visual features are concatenated with the textual features, after adding two special [CLS] and [SEP] tokens to mark the begnning and the ending of the textual input, and passed through the fusion encoder.

The model is pretrained on two objective, masked language modeling (MLM) and image-text matching. For both pretraining objective only a hundred random features are selected from the visual features instead of using the entire feature vector. For MLM language tokens are randomly masked with a probability of 15\% and the model is required to predict the masked token given the remaining language tokens and the sampled feature tokens. The other training objective is image-text matching, where the model perform a binary classification on whether the given image and text pair match each other or not.
For the downstream tasks, the random visual features sampling is not used, the entire feature vector is concatenated with the language tokens.

\subsubsection{ViTCAP}
ViTCAP \cite{} is an image encoder and fusion decoder architecture, which aims at mimicking the information obtained by detection-based architecture through the usage of a small auxiliary network called concept token network (CTN). The model uses vanilla transformer architecture for all the encoder, the auxiliary network and the fusion decoder. 

For the CTN, the network consists of a  transformer block, where the intermediate output of the vision encoder is used as an input to it. The network is trained in a multi-label classification manner using the CLS token of the transformer block. The pesudo-labels are constructed either by using library such as NLTK to extract the nouns in the captions, or retrieved from a detection model. To negate the imbalance in the extracted labels, asymmetrical focal loss is used instead of cross entropy. The input to the fusion decoder is then the concatenation of the top-K outputs of the CTN (where K is a hyperparameter) and the visual features, where the model is trained with an auto-regressive language model task. To further improve the performance, the authors employed knowledge distillation by using VinVL \cite{vinvil} as the teacher model and apply kullback leibler divergence on the output probabilities of both model.

The model achieves competitive results in image captioning and novel object captioning, but still slightly inferior to models that employs detection regions as an input to the vision encoder.

\subsubsection{KOSMOS-1}
KOSMOS \cite{} is an image encoder fusion decoder architecture that is similar to \cite{alayrac2022flamingo} takes text interleaved with image input. But unlike flamingo, the model employs merged attention, where the text and image tokens are passed to the decoder as one sequence. The image encoder is a pre-trained CLIP ViT-L/14 \cite{radford2021learning} (which is frozen except for the last layer) with a resampler \cite{alayrac2022flamingo} to reduce the emeddings size, and the fusion decoder is a pretrained Magneto \cite{}.

Kosmos was trained on uni-modal, cross-modal paired data, and interleaved multi-modal data. The input have a general format where the sequence starts and ends with the tokens <s> and </s> and a special token is used to indicates the start and end of an image tokens as "<image> visual embedding </image>". The pretraining datasets include: the pile\cite{}, common crawl \cite{} for uni-modal pretraining and LAION-2B\cite{}, LAION-400M\cite{}, COYO-700M\cite{} and Conceptual Captions\cite{} for multi-modal pretraining. In addition to a huge interleaved image-text data crawled from the web. The model is trained in a language model auto-regressive manner, given the visual tokens and the predicted text tokens the model predicts the next token. The loss is only calculated on the discrete tokens e.g. text tokens.

After pre-training, the model is further fine-tuned using language-only instruction tuning.
the model is given instruction data in the format of (instructions, inputs and outputs), and the model is trained in as a language modeling task. Both Unnatural instructions and FLANv2 instructions are used as the instruction dataset.

The model achieves a state of the art performance on several zero-shot tasks including image captioning and VQA, while having relatively fewer parameters. Furthermore, the model exhibit reasoning capabilities shown in the performance on Raven’s Progressive Matrices \cite{}. One interesting case in the training tasks was in image classification, the model was pretrained on image labels with description instead of only labels. The resulted in a significant improvement in the classification accuracy.

\subsubsection{PaLI: A Jointly-Scaled Multilingual Language-Image Model}
PaLI \cite{} is a massive dual encoders single decoder architecture that perform really well on various uni-modal and multi-modal tasks in different languages. The image encoder is an enormous 4 billion parameter ViT \cite{dosovitskiy2020image} dubbed e-ViT trained from scratch on JFT-3B dataset, while the encoder-decoder architecture follow mT5-XXL \cite{}. Both text inputs and the visual features extracted via the encoder are passed through the transformer encoder which in turns feeds its output to the transformer decoder. Unlike the text encoder-decoder, the vision encoder is frozen during pretraining.
A wide range of uni-modal and multi-modal datasets are used for pretraining including: WebLI (which is a massive alt-text data scrapped from the web and cleaned rigorously), Conceptual Captions 3M, WebLI OCR-text data (a generated ocr dataset from WEbLI using GCP Vision API), $VQ^2A-CC3M$, Open Images, Visual Genome, Object365 and WebLi corpus. Most of the datasets are machine translated into 35 language and further used for training.

The model is pretrained on several tasks, including uni-modal text task in order to negate catastrophic forgetting and maintain the fluency of the language model. All of the pretraining task are constructed as language modeling where the model perdicts tokens auto-regressively. The pretraining tasks include: Span corruption on text-only data, SplitCap, image Captioning, OCR, English and Cross-Lingual visual question answering (VQA),  English and Cross-Lingual visual question generation (VQG),  English-only Object-Aware VQA,  Object detection. Although the model achieves state-of-the-art results on various benchmarks, it relays heavily on custom input prompts, complex sometimes, where every task is formulated as "image+query to answer", not to mention the massive size of the model, which makes it less practical in real world scenarios.

\subsubsection{VL-ADAPTER: Parameter-Efficient Transfer Learning for Vision-and-Language Tasks}
The authors study the effect of utilizing adapter against  fine-tuning of vision language models. The adapters used in the study are the vanilla adapter, hyperformer and compacter. Experiments were done on a model with clip as the vision encoder \cite{} and BART\cite{lewis2019bart}/T5 as the text decoder. 

The adapters were inserted after each self-attention and fully connected layer in the text decoder, Inserting them in the vision encoder did not improve performance.  The authors experimented with three variation for each of the three adapters: single adapter for all taxes, half shared adapters and multiple adapters for each task. The vanilla single adapter resulted in the best performance across all tasks. Further more, the authors experimented with freezing different part of the model which gave the following observations: The performance of a frozen clip surpasses both trainable and clip with adapter layers. Unfrozen layer-normalization in the text decoder achieves better performance than freezing the entire decoder with very little added parameters. Adding adapters in the text decoder results in better performance comapred to finetuning the entire decoder.
\subsubsection{Donut:OCR-free Document Understanding Transformer}
Donut uses a simple image encoder and a transformer decoder for the task of document understanding. The image encoder is SWIN \cite{liu2021swin} transformer, while the text decoder is BART model \cite{BART}. The model is pretrained in an auto regressive manner where the model predicts the next text token given the previous token and image 

\subsection{Instruction Tuning}
Recent models attempt to give VLMs conversational abilities as well as more fluency in generation by exploiting instruction fine-tuning. Instruction finetuning is achieved by creating a fine-grained dataset usually using human annotators that instruct the model to generate text directed to solve a specific task. 

\subsubsection{LLaVA: Large Language and Vision Assistant}
LLaVA experiments with using instruction finetuining on large vision language models. The model was instruction fintuned on a dataset of 158K text-image pairs created using GPT-4. The architecture consists of  CLIP ViT-L/14 as the image encoder and LLaMA as the text decoder. In addition to a trainable projection matrix that is used to project the image features to a dimension compatible with the input to the text decoder.
The model is finetuned in two stages: The first stage is to align the visual and textual features via training the projection matrix. Both the vision encoder and text decoder are frozen, while the projection matrix is the only trainable parameters. The dataset used for training is a 595K image-text pair filtered from CC3M, the data is preprocessed in a similar fashion to the instruction data. For the second pretraining stage, the model is further fine-tuned using 158k language-image instruction following data. Only the vison encoder is frozen, while both the text decoder and projection matrix are trainable. During training the second stage, the data is constructed in a multi-turn conversation manner where a question (instruction) and its answer is randomly choses each turn. Each conversation can be one or more turns. The auto-regressive training objective, conditioned on the visual features, is used for both training stages.

For the instructions-following data, instead of the simple approach where GPT-4 is given an image and guided to provide an answer, the authors used the language-only GPT-4 in order to get more diverse responses and in-depth reasoning. In order to provide the visual cues for the language-only GPT4, The image is encoded into a format mentioning the objects in the image and their bounding box coordinates. In addition, the captions of the image is also provided in the prompt.

